Taqyim: Evaluating Arabic NLP Tasks Using ChatGPT Models

Large language models (LLMs) have demonstrated impressive performance on various downstream tasks without requiring fine-tuning, including ChatGPT, a chat-based model built on top of LLMs such as GPT-3.5 and GPT-4. Despite having a lower training proportion compared to English, these models also exhibit remarkable capabilities in other languages. In this study, we assess the performance of GPT-3.5 and GPT-4 models on seven distinct Arabic NLP tasks: sentiment analysis, translation, transliteration, paraphrasing, part of speech tagging, summarization, and diacritization. Our findings reveal that GPT-4 outperforms GPT-3.5 on five out of the seven tasks. Furthermore, we conduct an extensive analysis of the sentiment analysis task, providing insights into how LLMs achieve exceptional results on a challenging dialectal dataset. Additionally, we introduce a new Python interface https://github.com/ARBML/Taqyim that facilitates the evaluation of these tasks effortlessly.

==> related_work_section.tex <==
% This section summarizes the recent work with ChatGPT


\section{Related Work}

\paragraph{Large Language Models.} 
% Badr removed this: These models follow pre-training and fine-tuning learning paradigm \cite{zhao2023survey}

Several language models have been proposed recently. One of the earliest pre-trained language models is ELMo which was proposed to model the word context \cite{peters-etal-2018-deep}. ELMo learns the word context by pre-training a two-layer bidirectional LSTM network on large data and fine-tuning it on downstream tasks. BERT followed this learning strategy with a Transformer model pre-trained on large datasets \cite{Devlin2019BERTPO}. The performance of BERT outperformed other models on several downstream tasks. This learning paradigm motivated researchers to propose either new architectures (e.g., BART \cite{lewis2019bart} and GPT-2 \cite{radford2019language}) or enhanced pre-training techniques \cite{liu2019roberta, sanh2021multitask, wang2022language}. Scaling language models in terms of model size or data used for model pre-training has shown its effectiveness in several downstream tasks \cite{zhao2023survey}. This led to the introduction of the “large language models (LLM)” term. These models are trained on large datasets and usually have billions of parameters. Such LLMs showed a better performance compared with the smaller models with similar architectures and pre-training tasks (e.g., GPT-3 \cite{brown2020language} vs GPT-2).  Recently, a significant number of LLMs have been introduced, such as GPT-3, LLaMA \cite{touvron2023llama}, PaLM \cite{chowdhery2022palm}, T5 \cite{raffel2020exploring}, BLOOM \cite{muennighoff2022crosslingual}, and Chinchilla \cite{hoffmann2022training}. ChatGPT\footnote{ \url{https://openai.com/blog/chatgpt}} is one of these LLMs that was developed based on the GPT model series (GPT-3.5 and GPT-4) and showed a powerful performance with dialogue tasks. 

\paragraph{ChatGPT Evaluation} 
Following the introduction of ChatGPT, numerous studies have emerged assessing its performance across diverse tasks, encompassing machine translation \cite{jiao2023chatgpt, hendy2023good}, reasoning \cite{bang2023multitask, qin2023chatgpt}, the health care domain \cite{SLAPETA2023314, medicalchatgpt2023}, among others \cite{liu2023summary}. In one investigation, \citet{bang2023multitask} comprehensively assessed the performance of ChatGPT on eight distinct NLP tasks, employing a diverse set of 23 datasets. These tasks primarily revolved around the English language, with the exception of machine translation. The findings of this study unveiled that ChatGPT outperformed several state-of-the-art models across various NLP tasks. However, certain limitations were observed in specific scenarios, such as summarization, machine translation, particularly for low-resource languages, and reasoning capabilities.

Conversely, \citet{qin2023chatgpt} conducted an investigation revealing ChatGPT's robust performance in numerous NLP tasks, particularly highlighting its proficiency in reasoning tasks. However, the model exhibited limitations in certain tasks, such as sequence tagging. Furthermore, \citet{chan2023chatgpt} evaluated ChatGPT's capabilities in capturing inter-sentential relations, including discourse, causal, and temporal relationships. The reported outcomes demonstrated ChatGPT's adeptness in identifying and reasoning causal relationships. Conversely, the model's performance proved to be sub-optimal in tasks related to dialogue discourse parsing and detecting temporal relationships between two events. Notably, ChatGPT exhibited satisfactory detection of explicit discourse relations, yet encountered difficulties in handling implicit discourse relations.

% \citet{bang2023multitask} evaluated the performance of ChatGPT on eight NLP tasks using 23 datasets. Almost all these tasks are related to the English language, except machine translation. The results of this study reveal that ChatGPT outperformed several SoTA models on different NLP tasks. However, some failure cases have been observed with some tasks, such as summarization, machine translation, especially with low-resource languages, and reasoning. In contrast, \citet{qin2023chatgpt} found that ChatGPT exhibits strong performance on several NLP tasks favoring reasoning capabilities while it was not proficient in solving some tasks, such as sequence tagging. 
% \citet{chan2023chatgpt} also evaluated ChatGPT on inter-sentential relations, such as discourse, causal, and temporal relations. The reported results show that ChatGPT performed well in identifying and reasoning causal relations, whereas its performance was poor in the dialogue discourse parsing task and in detecting temporal relationships between two events. In addition, ChatGPT was able to detect most discourse relations with explicit discourse connectives and it failed with implicit discourse relations. 

% \citet{tawkat2023gptaraeval} conducted a technical evaluation of ChatGPT on various Arabic natural language understanding and generation tasks. The authors compared the performance of ChatGPT with BLOOMZ \cite{bloom} and AraT5 LLMs. The reported results show that ChatGPT can struggle on multiple Arabic tasks under few-shot learning compared to AraT5. The extensive evaluation by \citet{abdelali2023benchmarking} on many Arabic NLP tasks also showed that ChatGPT underperforms the SoTA models in the majority of the evaluated tasks.  

\paragraph{Concurrent Work}
During the course of our study, two papers have been published that evaluate ChatGPT models across multiple Arabic NLP tasks. Namely, \citet{tawkat2023gptaraeval} evaluated GPT-3.5 on a variety of Arabic NLU \cite{Elmadany2022ORCAAC} and NLG tasks, and compared it against the multilingual BLOOMZ ($7.1$B) model \cite{muennighoff2022crosslingual} and the much smaller monolingual AraT5 \cite{elmadany2022arat5} fine-tuned on each respective task. Their evaluation encompassed varying numbers of few-shot demonstrations within the context, with $\textsc{n-shot}=\{0, 3, 5, 10\}$. Their results demonstrated that while GPT-3.5 exhibited superior performance compared to BLOOMZ on Arabic tasks, it still significantly trailed behind the smaller-scale, Arabic-specific finetuned model, AraT5. In another related study, \citet{abdelali2023benchmarking} conducted an evaluation of GPT-3.5 on a range of Arabic NLP and Speech processing tasks. However, their investigation lacked explicit disclosure to some of their evaluation methodology (e.g. on the diacritization task), hindering the reproducibility of their findings. In contrast, our research provides comprehensive and transparent documentation of all pertinent details. Additionally, we extend the evaluation to include GPT-4 and provide additional analysis to the models' outputs in Section \ref{sec:analysis}.

==> tables/fewshots.tex <==
\begin{table}[]
\begin{tabular}{lllll}
\hline
fewshots & 0     & 3     & 5     & 10    \\ \hline
GPT-3.5  & 86.94 & 80.83 & 85    & 84.19 \\ \hline
GPT-4    & 91.14 & 92.83 & 95.37 & 92.30 \\ \hline
\end{tabular}
\caption{Few-shot results on both. models\label{tab:fewshot_results}}

\end{table}
